ExpRDiff: Short-exposure Guided Diffusion Model for Realistic Local Motion Deblurring

Removing blur caused by moving objects is challenging, as the moving objects are usually significantly blurry while the static background remains clear. Existing methods that rely on local blur detection often suffer from inaccuracies and cannot generate satisfactory results when focusing solely on blurred regions. To overcome these problems, we first design a context-based local blur detection module that incorporates additional contextual information to improve the identification of blurry regions. Considering that modern smartphones are equipped with cameras capable of providing short-exposure images, we develop a blur-aware guided image restoration method that utilizes sharp structural details from short-exposure images, facilitating accurate reconstruction of heavily blurred regions. Furthermore, to restore images realistically and visually-pleasant, we develop a short-exposure guided diffusion model that explores useful features from short-exposure images and blurred regions to better constrain the diffusion process. Finally, we formulate the above components into a simple yet effective network, named ExpRDiff. Experimental results show that ExpRDiff performs favorably against state-of-the-art methods.

==> sec/0_abstract.tex <==
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\vspace{-10mm}
\begin{center}
    % \hspace{-10mm}
    \includegraphics[width=1\linewidth, height=0.27\textheight]{fig/fig222.pdf} \\ % 替换为你的单幅图像路径
    \vspace{-3mm}
    \captionof{figure}{ of the proposed method } 
    \vspace{1mm}
    \label{fig:potential}
\end{center}%
}]


\begin{abstract}
%
Removing blur caused by moving objects is challenging, as the moving objects are usually significantly blurry while the static background remains clear.
%
Existing methods that rely on local blur detection often suffer from inaccuracies and cannot generate satisfactory results when focusing solely on blurred regions.
%
% To overcome this problem, We propose a simple yet effective Diffusion-based Local Deblurring Network (DLDNet) that restores local motion blurring by using short-exposure images as reference images.
%
To overcome these problems, we first design a context-based local blur detection module that incorporates additional contextual information to improve the identification of blurry regions.
%
Considering that modern smartphones are equipped with cameras capable of providing short-exposure images, we develop a blur-aware guided image restoration method that utilizes sharp structural details from short-exposure images, facilitating accurate reconstruction of heavily blurred regions.
%
Furthermore, to restore realistic images with better visually pleasant quality, we develop a short-exposure guided diffusion model that explores useful features from short-exposure images and blurred regions to better constrain the diffusion process.
%
Finally, we formulate the above components into a simple yet effective model, named as \ournet, to restore high-quality images. 
%
Experimental results show that \ournet performs favorably against state-of-the-art methods.
% %
% Removing blur caused by moving objects is quite challenging， as the moving objects are blurry while the static background is images clear. 
% %
% Relying on local blur detection does not generate favorable results. 
% %
% Existing camera provide short-exposure images, which can help blur removal. 
% %
% We propose a simple yet effective Diffusion-based Local Deblurring Network (DLDNet) that restores local motion blurring by using short-exposure images as reference images.
% %
% To enable the network to focus on blurry regions, we design a Context-based Local Blur Detection Module (CLBDM) that identifies blurry regions and generates blurred regions mask.
% %
% However, as the blur caused by the motion of objects is usually significant, focusing the network only on the blurred region cannot improve the reconstruction ability of the network for the blurred region.
% %
% Therefore, we first develop a blur-aware guided image restoration method that utilizes sharp structural details from short-exposure reference images, facilitating accurate reconstruction of heavily blurred regions. 
% %
% To further enhance the reconstruction capabilities of diffusion priors in blurred regions, we develop a Short-Exposure Guided Diffusion Model (SEGDM) that leverages short-exposure images and blurred regions mask to guide the diffusion process, thereby strengthening the effect of diffusion priors in blurred regions.
% %
% Experimental results show that our method has surprising performance in the restoration of locally blurred images caused by the object motion taken by a mobile phone compared to the existing state-of-the-art methods.
%Removing blur caused by moving objects is quite challenging as the moving objects are blurry while the static background is images clear. Relying local blur detection does not generate favorable results. Existing camera providing short-exposure images, which can help blur removal. We 
\end{abstract}



% %
% Our work is motivated by the fact that existing local deblurring methods can restore locally blurred images, yet due to the limitation of their dataset creation process, the image has a slight blur and the scenes of locally blurred images are mostly well lit, which makes the method trained on those datasets have poor restoration of locally blurred images with heavy blur in complex scenes, such as in dark-light conditions. 
% %
% Moreover, existing deblurring networks have poor performance for deblurring with heavy blur.
% %
% To overcome this problem, we design a blur detection module that generates a mask of the blurred area, followed by the use of a mask guided filter to allow blurred images to obtain sharp structural information from the blurred area corresponding to short-exposure images, which can be used to help restore heavily blurred areas with more loss structures.
% %
% After that, we define a blur mask splicing self-attention module to better utilize the prior of diffusion to restore the lost information of the blurred area in complex scenes.
% %





% Experimental results show that our method has surprising performance in the restoration of locally blurred images caused by the object motion taken by a mobile phone compared to the existing state-of-the-art methods.







% %
% Removing blur caused by moving objects is challenging, as the moving objects are usually significantly blurry while the static background remains clear.
% %
% Existing methods relying on local blur detection struggle with inaccuracies and cannot improve the reconstruction ability by only focusing on blurred areas.
% %
% To overcome this problem, We propose a simple yet effective Diffusion-based Local Deblurring Network (DLDNet) that restores local motion blurring by using short-exposure images as reference images.
% %
% Specifically, we design a Context-based Local Blur Detection Module that incorporates additional contextual information to improve the identification of blurry regions.
% %
% Considering that modern smartphones are equipped with cameras capable of providing short-exposure images, we develop a blur-aware guided image restoration method that utilizes sharp structural details from short-exposure reference images, facilitating accurate reconstruction of heavily blurred regions.
% %
% Finally, to achieve realistic reconstruction results in blurred regions, we develop a Short-Exposure Guided Diffusion Model (SEGDM), which utilizes short-exposure images and blurred region masks to guide the diffusion process.
% %
% Experimental results show that our method performs favorably against the existing state-of-the-art methods.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
%
%Currently, handheld devices such as HUAWEI Mate XT and Insta 360 are equipped with their own hardware anti-shake motors, masking it unlikely that the captured images contain global blur.
%
%However, the blurring caused by object motion still exists when capturing photos with these devices, and this localized blurring is more extensive in low-light conditions.
%
%Therefore, it is necessary to restore the locally blurred image in low-light conditions so that it can be pleasantly viewed on social networks.
%
Existing smart phones equipped with anti-shake functions significantly improve the quality of captured images. However, capturing clear moving objects in a dynamic low-light environment is still a difficult problem as a longer exposure time is often required and the speed of the moving objects is fast. The captured images usually contain significant local blur effect; e.g., the objects are blurry while the static background is usually clear. Thus, how to deblur images with the local blur effect receives significant attention from both academic and industry communities. 

%
Most existing methods are designed mainly for images with a uniform or non-uniform global blur effect~\cite{MIMO, Deeprft, MPRNet, NAFNet, Uformer, Fftformer, Stripformer, Restormer}. When applying these methods to images with local blur, the clear background will be oversmoothed, while moving objects are not restored well. Thus, it is of great need to develop an effective method to handle the clear background and blurry objects simultaneously for better image restoration. 

To this end, several approaches~\cite{RoLeBlur, LMD-ViT} usually adopt object segmentation or blur detection approaches to differentiate between blurry and clear regions, subsequently handling blur regions and clear regions simultaneously. However, localized blurs resulting from object motion often present significant challenges, and adverse imaging conditions, such as low-light environments, further increase the difficulty of object segmentation or blur detection. As a result, reliance solely on object segmentation or blur detection does not effectively improve deblurring performance. 

%In addition, these blur detection methods are based on pixel-wise classification, which is less effective .  
We note that existing handheld devices can capture multiple photos of a moving object simultaneously through burst mode or multi-camera systems. Photos captured using these settings typically contain sharp details due to the short exposure times. Thus, it is of great interest to explore the information of these images to facilitate local blur removal.

%Existing image deblurring methods~\cite{MIMO, Deeprft, MPRNet, NAFNet, Uformer, Fftformer, Stripformer, Restormer} based on deep convolutional neural networks (CNNs) and transformers exhibit impressive reconstruction performance in globally blurred images. 
%
%However, these methods inevitably process clear regions within locally blurred images, leading to the loss of high-frequency details in those areas.
%
%To address the above problem, existing local motion deblurring methods~\cite{RoLeBlur, LMD-ViT} aim to reduce the network's processing of clear regions by employing methods to detect blurred areas.
%
%However, localized blurring caused by object motion is typically substantial, and simply utilizing blur detection does not enhance the subsequent deblurring effectiveness for larger blurs within the mask.
%
%Furthermore, these blur detection methods are based on single-pixel classification, which can lead to low prediction accuracy.
%

%
%As existing handheld devices can capture multiple images of a moving target simultaneously through burst mode or multi-camera systems, it becomes relatively easy to obtain reference images of the subject.
%
%Given the photographer's high-quality expectations for the captured images, it is essential to explore how to leverage reference images better to restore locally blurred images.
%

%
To solve the problems mentioned above, we develop a \ournet to explore information from localized blur regions and short-exposure images as guidance to facilitate local blur removal.
%
First, given that not all the regions of captured images are blurry, we develop a context-based local blur detection module (CLBDM) to explore contextual information for better identification of the blurry regions.
%
Then, we develop a simple yet effective blurry-aware guided image restoration that explores the useful information of short-exposure images and the detected blurry regions as guidance to discriminately handle the blurry regions and clear regions simultaneously for better image restoration. 
%

However, as the moving speeds of the objects are usually fast, which leads to significant blur effects, restoring realistic clear images with rich details from heavily blurred images is not a trivial task. 
%
%However, as the blur caused by the moving objects is usually significant, restoring clear images with better structural details is not a trivial task. 
%
%thus, we develop a blurry-aware guided image restoration method, where the detected blurry regions and short-exposure images are used to guide the clear image restoration. 
%
Motivated by the success of diffusion-based methods~\cite{SUPIR, PASD} in high-quality image generation, we take advantage of diffusion priors to help realistic clear image restoration. 
%
To ensure that the diffusion model pays more attention to restoring reliable structural details, we develop a simple yet effective feature fusion method, named ExpBFusion, to adaptively extract useful features from the short-exposure images and the detected blurry regions. These features obtained through ExpBFusion can then guide the diffusion model for better image restoration. 
%

By formulating the aforementioned modules into a unified framework, the proposed \ournet achieves favorable performance against state-of-the-art methods on publicly available local blur datasets as well as real-world scenarios. 
%
% Then, with the detected blurry regions, we develop a mask guided image restoration method to obtain initial deblurred results under the guidance of 
%
%Inspired by recent diffusion-based image restoration methods~\cite{SUPIR, PASD} utilize clearer conditions to guide the restoration process, resulting in more photorealistic outcomes, we use the prior of diffusion to restore the locally blurred image.
%
% %
% With the rapid development of diffusion probabilistic denoising models (DDPMs), a series of diffusion-based image restoration methods~\cite{DiffBIR, FeMaSR, StableSR} have achieved surprisingly impressive performance on real-world data.
% %
% Inspired by the structure of ControlNet, DLDN employs RealVisXL, which is a variant of StableDiffusion-XL (SDXL)~\cite{SDXL} aimed at photorealism.
% %
%
%In order to enhance the focus on blurred areas during the diffusion-based image generation process and to procure more accurate structural information from the short-exposure images, we propose a blur mask splicing self-attention module (BMSSAM) that employs a blur mask as an additional conditional input.
%
%Furthermore, we leverage an adapter to extract and integrate features from the short-exposure images into the UNet at various spatial scales, thereby facilitating the diffusion model's ability to refine the blurred areas with greater precision.
%

% %
% Additionally, in order to more effectively remove blur in real-world scenarios, we created a dataset of real-world low-light images with local blur from long- and short-exposure image pairs. 
%
%Our method achieves competitive results on this dataset, demonstrating the capability to remove blur present in long-exposure images genuinely.

%
The main contributions are summarized as follows.
%
\begin{itemize}
    \item We develop a context-based local blur detection module to explore additional contextual information to improve the identification of blurry regions.
    \item We develop a blurry-aware guided image restoration to remove local blur by handling the blurry regions and clear regions discriminately in the restoration process.
    \item We develop a short-exposure guided diffusion model to explore useful features from the short-exposure images and the detected blurry regions as guidance for realistic image restoration. 
\end{itemize}
\vspace{5mm}
%

% \section{Introduction}
% \label{sec:intro}
% % %
% % Image deblurring is a challenging task for restoring the sharp image from the blurred ones.
% % %
% % With the rapid growth of the demand for handheld recording devices and the booming outdoor self-media field, photo quality has attracted significant attention.
% % %
% % However, the object motion and camera shake usually lead to significant blur effects when taking photos with handheld devices. 
% % %
% % Thus, it is necessary to restore a sharp image from a blurred image so that it can pleasantly be viewed on social media.
% %

% %
% Currently, handheld devices such as HUAWEI Mate XT and Insta 360 are equipped with their own hardware anti-shake motors, masking it being unlikely that the captured images contain global blur.
% %
% However, the blurring caused by object motion still exists when capturing photos with these devices, and this localized blurring is more extensive in low-light conditions.
% %
% Therefore, it is necessary to restore the locally blurred image in low-light conditions so that it can be pleasantly viewed on social networks.



% % %
% % In previous methods, Joint filter-based methods such as joint bilateral and guided image filters can restore degraded images with reference images.
% % %
% % These methods make an assumption that the reference images have correct structural information that effectively guides the restoration process.
% % %
% % However, photos taken with different cameras can not provide pleasant reference images due to different resolutions or exposure times.
% % %
% % \cite{CFJIRVSM, MSJF} utilized valid information of both reference images and degraded images to jointly image restoration.
% % %
% % Hand-crafted prior-based deburring methods~\cite{RDMD, RFD, IDBNIP} make an adequate to joint image deblurring using two different degraded images, still, these methods usually estimate blur kernel under some assumed priors that lead to complex scenarios that are difficult to solve.



% % %
% % In the past period, deep learning has witnessed significant development in the field of computer vision.
% % %
% % deep convolutional neural networks (CNNs) based image deblurring methods~\cite{MIMO, Deeprft, MPRNet, NAFNet} achieve impressive reconstruction performance.
% % %
% % Transformer-based methods~\cite{Uformer, Fftformer, Stripformer, Restormer} rely on the capabilities of exploring non-local information to achieve better performance than CNN-based methods.
% % %
% % The CNN-based method\cite{SelfIR} simulates long-exposure blur images and short-exposure noise images and utilizes an unsupervised for image restoration jointly.
% % %
% % However, the dataset does not include local blurring caused by object motion, leading to a lack of detail in the clear areas of the recovered image.
% % %
% % \cite{RoLeBlur} employs a dual-camera system combined with a beam splitter to capture data pairs consisting of local blur caused by object motion and their corresponding clear images. Additionally, a blur detection module is used to generate a mask that serves as prior information for the deblur network.
% % %
% % The dual-camera method requires high-quality short-exposure images as ground truth, which makes it challenging to obtain real-world blurring training data pairs in low-light conditions.
% % %
% % All of these methods have difficulty dealing with heavy blurs.
% % %

% %
% Existing image deblurring methods~\cite{MIMO, Deeprft, MPRNet, NAFNet, Uformer, Fftformer, Stripformer, Restormer} based on deep convolutional neural networks (CNNs) and transformers exhibit impressive reconstruction performance in globally blurred images. 
% %
% However, these methods inevitably process clear regions within locally blurred images, leading to the loss of high-frequency details in those areas.
% %
% To address the above problem, \cite{RoLeBlur} employs a dual-camera system combined with a beam splitter to capture data pairs consisting of local blur caused by object motion and their corresponding clear images. 
% %
% Additionally, a blur detection module is used to generate a mask that serves as prior information for the deblur network.
% %
% However, the dataset requires high-quality short-exposure images as ground truth, which makes it challenging to obtain real-world heavy blurring training data pairs.
% %
% This is because short-exposure images typically contain significant noise in low-light conditions.
% %
% Consequently, models trained on such datasets struggle to effectively restore the latent sharp image from the locally blurred image with insufficient light.
% %
% To overcome this problem, the CNN-based method\cite{SelfIR} simulates long-exposure blur images and short-exposure noise images and utilizes an unsupervised for image restoration jointly.
% %
% However, this approach does not consider local blurring and the captured data lack a reliable ground truth.
% %


% % The CNN-based method\cite{SelfIR} simulates long-exposure blur images and short-exposure noise images and utilizes an unsupervised for image restoration jointly.
% % %
% % However, the dataset does not include local blurring caused by object motion, leading to a lack of detail in the clear areas of the recovered image.
% % %
% % \cite{RoLeBlur} employs a dual-camera system combined with a beam splitter to capture data pairs consisting of local blur caused by object motion and their corresponding clear images. Additionally, a blur detection module is used to generate a mask that serves as prior information for the deblur network.
% % %
% % The dual-camera method requires high-quality short-exposure images as ground truth, which makes it challenging to obtain real-world blurring training data pairs in low-light conditions.
% % %
% % All of these methods have difficulty dealing with heavy blurs.
% % %

% % %
% % With the rapid development of denoising diffusion probabilistic models (DDPMs), a series of diffusion-based image restoration methods~\cite{DiffBIR, FeMaSR, StableSR} have achieved surprisingly impressive performance on real-world data.
% % %
% %

% %
% In this paper, we develop a diffusion-based local motion deblurring network (DLDNet) that aims to restore local motion-blurred images with heavy blur in a complex environment.
% %
% First, to enable the network to focus more on restoring blurred areas, we design a domain blur detection module (DBDM) that generates a blur mask using long-exposure images with local blur.
% %
% Subsequently, we use the corresponding short-exposure images as guided images to perform guided filtering within the mask area.
% %
% With the rapid development of diffusion probabilistic denoising models (DDPMs), a series of diffusion-based image restoration methods~\cite{DiffBIR, FeMaSR, StableSR} have achieved surprisingly impressive performance on real-world data.
% %
% Inspired by the structure of controlnet, DLDN employs RealVisXL, which is a variant of StableDiffusion-XL (SDXL)~\cite{SDXL} aimed at photorealism.
% %
% In order to enhance the focus on blurred areas during the diffusion-based image generation process and to procure more accurate structural information from the short-exposure images, we propose a blur mask splicing self-attention module (BMSSAM) that employs a blur mask as an additional conditional input.
% %
% Furthermore, we leverage an adapter to extract and integrate features from the short-exposure images into the UNet at various spatial scales, thereby facilitating the diffusion model's ability to refine the blurred areas with greater precision.
% %

% %
% Additionally, in order to more effectively remove blur in real-world scenarios, we created a dataset of real-world low-light images with local blur from long- and short-exposure image pairs. 
% %
% Our method achieves competitive results on this dataset, demonstrating the capability to remove blur present in long-exposure images genuinely.
% %

% %
% The main contributions are summarized as follows.
% %
% \begin{itemize}
%     \item We develop a diffusion-based local motion deblurring network (DLDNet) that aims to restore local motion-blurred images in low-light conditions.
%     \item We design a domain blur detection module (DBDM) that generates a blur mask using long-exposure images with local blur.
%     \item We propose a blur mask splicing self-attention module (BMSSAM) to enhance the focus on blurred areas during the diffusion-based image generation process.
%     \item Our proposed method has achieved competitive results on real-world night-time local blur datasets.
% \end{itemize}
% \vspace{5mm}
% %

















==> sec/2_related.tex <==
%
\begin{figure*}[htbp!]
    \centering
 \includegraphics[width=1\textwidth]{fig/network/fig1_1.pdf}
 \vspace{-4mm}
 \caption{
 An overview of the proposed method DLDNet. $\mathcal{A}$ containing three residual blocks. $\mathcal{D}$ is the domain blur detection module, the structure of the $\mathcal{D}$ in supplemental material. the latent encoder is used to extract clean features of the $\mathcal{N}_{s}$. The MGF is the Mask Guided image filtering. The details of the structure of the DLDN are described in Section~\ref{sec:method}.}
 \label{fig: Network FlowChart}
\end{figure*}
%

%
\section{Related Work}
\label{sec:related}
%
{\flushleft \textbf{Hand-crafted prior-based methods.}} Since image deblurring is ill-posed, conventional methods usually use reference images with clearer structural information as effective priors to jointly solve image deblurring.
%
In~\cite{RDMD} Chen et al. propose joint image deblurring with two images with different levels of blurring. 
%
Zhuo et al.~\cite{RFD} and Yuan et al.~\cite{IDBNIP} to perform image deblurring with the help of Flash images and noisy images as reference images, in which the structure is clearer, respectively.
%
Although traditional joint image deblurring methods can achieve better results than traditional single-image deblurring methods,  traditional joint image deblurring methods assume that the blurring are global of these images can be well described by a single blur kernel result from camera shake and the scene is static.
%
These methods provide poor performance of deblurring in images with non-uniform blurring and blurred images caused by object motion.
%

%
{\flushleft \textbf{Deep learning-based methods.}}
%
To solve more complex image deblurring situations avoiding the limitations assumed in manually designing image priors, Deep learning-based image deblurring methods are explored to solve image deblurring.
%
Lost of sigle image deblurring methods ~\cite{SRN, DeblurGAN, DeblurGANv2, DMPHN, SAPHN, MIMO, Deeprft, Uformer, Stripformer} achieve favorable performance. 
%
Zamir et al.~\cite{MPRNet} propose a multi-stage progressive image deblurring method for restoration image at each stage that non-parameter sharing network is utilized in different stages to learn the deblurring function of the corresponding scales.
%
While this design achieves competitive performance, the complexity of the model thus becomes larger.
%
To reduce the parameters of the model, Chen et al.~\cite{NAFNet} propose a computationally efficient simple baseline, which considers the nonlinear activation functions to be non-essential and replaces them. 
%
But the amount of convolutional operations makes those CNNs-based methods only have the ability to capture localized information.
%

%
With the development of transformer~\cite{Transformer} in high-level vision tasks, whose ability to capture global contexts caught the attention to researchers. 
%
~\cite{Restormer} calculates channel attention and ~\cite{Fftformer} computes the dot-product attention on the spatial frequency domain separately, which reduces the complexity of computing the attention weights in the transformer.
%
~\cite{LMD-ViT} propose a window-based local motion deblurring vision transformer network, which employs the confidence predictor that constrains the output at the pixel level using the mask of gt to predict blur areas.
%
The confidence predictor network is trained in such kind of strategy that it leads to mask generation inaccurately.
%

%
{\flushleft \textbf{Diffusion-based image restoration.}}
%
With the surprising performance of SDXL in image image-generating field, it has been developed for image restoration.
%
To solve the problem of uncontrollable generation of images in the image generation task, ~\cite{T2I_adapter, controlnet} employ another branch to extract the features of the condition to control the final generated output.
%
Inspired by that, \cite{PASD, SUPIR, DiffBIR} utilize the degradation network to generate clear images or clear latent from the input degraded images, which is used to put into the denoise u-net and the controlnet to control the diffusion process and generate high-quality images.
% %
% \cite{SUPIR} utilize 20 million high-quality images which include a variety of degradation methods, yet limited by the fact that most of these data degradations are synthetic, the degradation Robust Encoder has not encountered real object motion.
%
Although the images recovered by those methods achieve pleasant visualization results, the training of these methods is based on a large collection of high-quality images and utilizes synthetic degraded images, which does not allow for the restoration of local blur caused by object motion.
%
In order to better utilize the prior provided by SDXL to recover local blur in the presence of a reference image, we propose the diffusion-based low-light local motion deblurring network.
%



==> sec/3_method.tex <==
%
\section{Proposed Method}
\label{sec:method}
%
% We aim to present a simple yet effective model ExpRDiff for realistic local motion deblurring. 
%
% We aim to present a diffusion-based local motion deblurring network that restores long-exposure local motion blurred 
% using short-exposure images as guidance.

% %
% We aim to present a diffusion-based local motion deblurring network that restores long-exposure local motion blurred 
% using short-exposure images as guidance.
% %
% Specifically, we first design a context-based local blur detection module (CLBDM) that uses long-exposure blurry images to generate a blur regions mask.
% %
% Following that, we utilize short-exposure images as reference images to guide blurry-aware guided image filtering with long-exposure local blurry images so that the blurry regions of long-exposure images can acquire sharp structural details from the short-exposure images.
% %
% To allow diffusion process to focus more on the blurring regions, we propose a short-exposure guided diffusion model (SEGDM) that uses the short-exposure images and blurry regions mask as conditions to guide the diffusion process to focus more on the blurring regions and acquire sharp structural information.
% %
% We further formulate the above modules into an end-to-end trainable diffusion-based network that jointly utilizes long-exposure local blurry images and short-exposure images for image deblurring.
% %
% In the following, we will explain the main ideas of each component in detail.
% %
%
The proposed \ournet aims to explore useful features from short-exposure images and blurry regions as guidance for local blur removal and realistic image restoration. It contains a context-based local blur detection module that is used to identify blurry regions by exploring contextual information, a blurry-aware guided image restoration that uses the short-exposure images and blurry regions to remove local blur, and a short-exposure guided diffusion model that is constrained by the features of short-exposure images and blurry regions for realistic image restoration. Figure~\ref{fig: Network FlowChart} shows the overview of the proposed \ournet. In the following, we explain each component in details. 

%
\begin{figure*}[htbp!]
    \centering
 \includegraphics[width=1\textwidth]{fig/network/fig1_3.pdf}
 \vspace{-4mm}
 \caption{
 Network details of the proposed Domain Blur Detection Module for detecting the blur area of the long-exposure blur images.}
 \label{fig: Network FlowChart3}
\end{figure*}
%

%
\subsection{Context-based local blur detection module}
%
Local blur detection is an essential step for handling images with local blur. Existing methods~\cite{RoLeBlur, LMD-ViT} usually treat this problem as a binary classification and employ a binary network to determine whether each pixel position is blurry or not.
%
However, this approach, which relies solely on individual pixel characteristics, often fails to capture contextual information, leading to inaccurate blur detection and subsequent degradation in overall result quality. 
%
To address this problem, we develop a simple yet effective context-based local blur detection method that incorporates additional contextual information to enhance the robustness of local blur detection.

%
Specifically, we first divide the input blurry images into $N$ non-overlapping patches $\{P_{i}\}^{N}_{i=1}$ with the unfolding operation from input blurry image $B$, where $P_{i} \in \mathbb{R}^{C\times60\times60}$.
%
Then, we develop a simple yet effective network $\mathcal{D}(\cdot)$ to estimate a set of confidence values $\{V_{i}\}^{N}_{i=1}$, $V_{i} \in \mathbb{R}^{C\times1\times1}$, from the input blurry image to discriminate whether the divided patches $\{P_{i}\}^{N}_{i=1}$ are blurry or not:
\begin{equation}
    V_{i} = \mathcal{S}\left(\frac{\mathcal{D}(P_{i}) + G_{i}}{\tau}\right),
\end{equation}
where $G_{i} = -\log\left(-\log(U_{i})\right)$, $\quad U_{i} \sim \text{Uniform}(0, 1)$, $\mathcal{S}(\cdot)$ denotes the Softmax operation, $\tau$ is the temperature parameter that controls the smoothness of the distribution, $G_{i}$ represents the Gumbel noise added for differentiable sampling~\cite{gumbelsoftmax}, and $U_{i}$ is a random variable sampled from a uniform distribution $\text{Uniform}(0, 1)$. The detailed network architecture is shown in Figure~\ref{fig: Network FlowChart3}.

We train the network $\mathcal{D}$ by minimizing the following Cross-Entropy loss function:
%
\begin{equation}
    \mathcal{L} = -\frac{1}{N} \sum_{i=1}^{N} \left[ V_{i} \log(M_{i}^{gt})) + (1 - V_{i})\log(1 - M_{i}^{gt}) \right],
     % \mathcal{L}_{D} = \sum_{i=1}^{n}CrossEntropy(V_{i}, M_{i}),
\end{equation}
%
where $M_{i}^{gt}$ denotes the ground truth confidence map that indicates the blur degree of the patch $P_i$. It is obtained by cropping the corresponding region from the ground truth blur confidence map $M^{gt}$ based on the spatial position of patch $P_{i}$.

As the confidence map is estimated in image patches, we employ the nearest-neighbor interpolation to obtain the pixel-level confidence map $M$ to discriminate the blurry regions and clear regions from input image:
\begin{equation}
\begin{split}
    &\Tilde{V}_i = \mathcal{U}(\mathcal{S}(V_i)), \quad C_{i} \in \mathbb{R}^{C\times60\times60}, \\
    &M = \mathcal{R}(\Tilde{V}_i),
    \end{split}
\end{equation}
where $\mathcal{U}(\cdot)$ denotes the nearest-neighbor interpolation operation, $\mathcal{R}(\cdot)$ denotes the folding operation. 


%apply a simple yet effective blur detection network $\mathcal{D}(\cdot)$ with Gumbel-Softmax~\cite{gumbelsoftmax} $\mathcal{G}$ (see Figure~\ref{fig: Network FlowChart} for the detailed network architecture) to map $\{P_{i}\}^{N}_{i=1}$ to a set of confidence vectors $\{V_{i}\}^{N}_{i=1}$, where $V_{i} \in \mathbb{R}^{C\times1\times1}$.
% indicates whether the corresponding patch contains blur.
% %
% To better identify whether each patch contains blurred regions
%
% To identify whether each patch contains a blur region, we feed $\{P_{i}\}^{N}_{i=1}$ into a simple yet effective blur detection network $\mathcal{D}(\cdot)$.
%
% The network ultimately maps $\{P_{i}\}^{N}_{i=1}$ to a set of vectors $\{V_{i}\}^{N}_{i=1}$, where $V_{i} \in \mathbb{R}^{C\times1\times1}$, and $V_{i}$ indicates whether the corresponding patch contains blur.
%
%The confidence vectors $V_{i}$ are computed as follows:
%

%
%where $\text{Softmax}(\cdot)$ denotes the Softmax function, $\tau$ is the temperature parameter that controls the smoothness of the distribution, 
% \begin{equation}
%      V_{i} = \text{Softmax}\left(\frac{\mathcal{D}(P_{i}) + G_{i}}{\tau}\right),
%      % V_{i} = \mathcal{G}(\mathcal{D}(P_{i})),
% \end{equation}
%
%To constrain $V_{i}$ reflects the presence of blur in the corresponding patch $P_{i}$, we generate the label vectors $\{M_{i}\}^{N}_{i=1}$ from ground-truth blur regions mask $M$ using the same transformations that we applied to generate $\{P_{i}\}^{N}_{i=1}$, followed by a MaxPooling.
%
% Then, we use the $\{P_{i}\}^{N}_{i=1}$ 
% %
% To constrain that $V_{i}$ reflects the presence of blur in the corresponding patch $P_{i}$, we further apply the same transformations to the mask of ground-truth blur regions $M$ as were applied to local blurry images of long exposure to obtain the label vectors $\{M_{i}\}^{N}_{i=1}$ that are used to constrain $\{V_{i}\}^{N}_{i=1}$, identify that they properly represent the blur characteristics of each patch $P_{i}$.
% %
%The loss function of training $\mathcal{D}$ is denoted by:
%
%\begin{equation}
%    \mathcal{L} = -\frac{1}{N} \sum_{i=1}^{N} \left[ V_{i} \log(M_{i})) + (1 - V_{i})\log(1 - M_{i}) \right],
     % \mathcal{L}_{D} = \sum_{i=1}^{n}CrossEntropy(V_{i}, M_{i}),
%\end{equation}
%
%where $\mathcal{L}$ denotes the Cross-Entropy Loss function that measures the difference between the confidence vectors $V_{i}$ and the corresponding ground truth mask patches $M_{i}$.
%

%
%In testing, if the patch $P_{i}$, contains blur regions, $V_{i}$ is assigned a value of 1; otherwise, it is assigned a value of 0. 
%
%which is denoted by:
%
%\begin{equation}
%    \begin{split}
%        &V_{i}=\left\{
%        \begin{aligned}
%        &0, \ \frac{\exp(V_{i})}{\sum_{j} \exp(V_{j})} < \beta, \\
%        &1, \ \frac{\exp(V_{i})}{\sum_{j} \exp(V_{j})} \geq \beta,
%        \end{aligned}
%        \right.
%    \end{split}
%\end{equation}
%
%where $\exp(\cdot)$ denotes the exponential function, $\beta$ represents the default threshold in $\mathcal{G}(\cdot)$, and the denominator $\sum_{j} \exp(\cdot)$ is the normalization term that ensures the output values sum to 1.
%
%After that, we obtain the predicated blurring region mask $M^{'}$ by interpolating each $V_{i}$ of $\{V_{i}\}^{N}_{i=1}$ to a resolution of 60 $\times$ 60 using nearest-neighbor interpolation and restore its spatial dimensions align with the long-exposure images.  
%

%
\subsection{Blurry-aware guided image restoration}
%
\label{sec:MGIF}
%
With the guidance of a short exposure image, one can use the guided filtering methods~\cite{GIF} to help eliminate blur. However, directly using~\cite{GIF} will smooth the clear background as shown in Figure~\ref{}. 
%
A natural solution to this problem is that we do not handle the clear regions of the input images. 
%
To this end,  we adopt a threshold based on the default value of the Gumbel-Softmax distribution to binarize M.
%
Then, we develop a blurry-aware guided restoration approach that formulates the guided filtering method as:
\begin{equation}
     H(\textrm{x}) = M(\textrm{x})(a_kR(\textrm{x})+b_k) + (1-M(\textrm{x}))B(\textrm{x}), \textrm{x} \in w_k, 
     \label{modified GF}
\end{equation}
where $a_k$ and $b_k$ are linear coefficients in an image patch $w_k$; $B(\textrm{x})$ and $R(\textrm{x})$ denote the input blurry image and short exposure image at pixel $\textrm{x}$.

The linear coefficients $a_k$ and $b_k$ can be obtained by solving the following optimization problem:
\begin{equation}
     \min_{a_k, b_k}\sum_{i\in w_{k}}(M(\textrm{x})(a_kR(\textrm{x})+b_k) + (1-M(\textrm{x}))B(\textrm{x})-B(\textrm{x})+\epsilon a^{2}_{k}),
     \label{objective function}
\end{equation}
where $\epsilon$ is a weight parameter. Similar to~\cite{GIF}, the solution of $a_{k}$ and $b_{k}$ can be obtained: 
% \begin{equation}
%     \begin{split}
%          & a_{k}=\frac{\frac{1}{\mid w \mid}\sum_{i\in w_{k}}I_{i}p_{i}M^{'}_{i}-\mu_{k}\overline{p}_{k}\overline{M^{'}}_{k}}{{\sigma_{k}M^{'}_{i}}^{2}+\epsilon}, \\
%          & b_{k}=\overline{p_{k}}-(1+a_{k}\overline{M^{'}}_{k})\mu_{k}+\overline{M^{'}}_{k}\mu_{k}, \\
%          &\overline{p}_{k}=\frac{1}{\mid w \mid}\sum_{i\in w_{k}}p_{i}, \\
%          &\overline{M^{'}}_{k}=\frac{1}{\mid w \mid}\sum_{i\in w_{k}}M^{'}_{i}, 
%          \label{eq:7}
%       \end{split}
% \end{equation}
\begin{equation}
    \begin{split}
         & a_k = \frac{\sum_{i \in w_k} M(\textrm{x}_i) (R(\textrm{x}_i) - B(\textrm{x}_i))}{\sum_{i \in w_k} M(\textrm{x}_i) R(\textrm{x}_i)^2 + \epsilon}, \\
         & b_k = \frac{\sum_{i \in w_k} M(\textrm{x}_i) (B(\textrm{x}_i) - a_k R(\textrm{x}_i))}{\sum_{i \in w_k} M(\textrm{x}_i)},
         \label{eq:7}
      \end{split}
\end{equation}

% \begin{equation}
%     a_k = \frac{\sum_{i \in w_k} M(\textrm{x}_i) (R(\textrm{x}_i) - B(\textrm{x}_i))}{\sum_{i \in w_k} M(\textrm{x}_i) R(\textrm{x}_i)^2 + \epsilon}
%     \label{eq:a_k_solution}
% \end{equation}

% \begin{equation}
%     b_k = \frac{\sum_{i \in w_k} M(\textrm{x}_i) (B(\textrm{x}_i) - a_k R(\textrm{x}_i))}{\sum_{i \in w_k} M(\textrm{x}_i)}
%     \label{eq:b_k_solution}
% \end{equation}

% where $\mu_{k}$ and $\sigma^{2}_{k}$ are the mean and variance of $I$.
%
Figure~\ref{} shows that the proposed method can remove local blur well while it does not smooth the details of clear regions. 
%The restored image can be obtained by:
%\begin{equation}
%    H_{i}=(a_{k}{N_{s}}_{i}+b_{k})M_{i}+(1-M_{i}){N_{s}}_{i},  \forall N_{s} \in w_{k},
%    \label{eq:8}
%\end{equation}

%
%We refer to the module by Eqs.~(\ref{eq:7}) and~(\ref{eq:8}) as the proposed SEGDM module and show the effectiveness of SEGDM in Section~\ref{ablation51}.
%

%% Visual Comparisons
\begin{figure*}[t]
	\footnotesize
	\begin{center}
		\begin{tabular}{c c c c c c c c}
        \multicolumn{3}{c}{\multirow{5}*[48pt]{
            \hspace{-2.5mm} \includegraphics[width=0.42\linewidth,height=0.245\linewidth]{fig/experiments/1/fullimage.pdf}}}
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/1/input.pdf}
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/1/ReLoBlur.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/1/MIMO-UNet.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/1/NAFNet.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/1/Restormer.pdf} 
              \\
    		\multicolumn{3}{c}{~}                                   
            & \hspace{-4.0mm} (a) LQ
            & \hspace{-4.0mm} (b) ReLoBlur~\cite{RoLeBlur} 
            & \hspace{-4.0mm} (c) MIMO-UNet~\cite{MIMO}
            & \hspace{-4.0mm} (d) NAFNet~\cite{NAFNet} 
            & \hspace{-4.0mm} (e) Restormer~\cite{Restormer} 
            \\		
    	\multicolumn{3}{c}{~}
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/1/MIMO-UNet-cat.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/1/NAFNet-cat.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/1/Restormer-cat.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/1/ours.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/1/gt.pdf}
            \\
    	\multicolumn{3}{c}{\hspace{-4.0mm} \textbf{Blurry input}}
            & \hspace{-4.0mm} (f) MIMO-UNet*~\cite{MIMO} 
            & \hspace{-4.0mm} (g) NAFNet*~\cite{NAFNet} 
            & \hspace{-4.0mm} (h) Restormer*~\cite{Restormer}
            & \hspace{-4.0mm} (i) our
            & \hspace{-4.0mm} (j) GT patch\\ 	 	
        
		\end{tabular}
	\end{center}
 
	\vspace{-6mm}
	\caption{Visual comparisons on challenging \textbf{coupled degradation} inputs from the proposed benchmark. Zoom in for a better view.}
	\label{fig:visual1}
	%\vspace{-2mm}
\end{figure*}

%
\subsection{Short-exposure guided diffusion model}
%
Although the proposed blurry-aware guided image restoration can remove local blur well, it is less effective to restore realistic images with details due to the significant blur caused by moving objects. 
%
We note that existing diffusion-based methods with text prompts can recover details from the degraded image.
%
However, text information is a high-level feature and cannot effectively characterize blurry regions and low-level structural features of images. Thus, only using the text prompt does not guide the diffusion models for realistic image restoration when local blur exists.
%
To address this problem, we propose a short-exposure guided diffusion model that explores the features of both short-exposure images and blurry regions for better image restoration.
%

%
\begin{figure}[tb]
    \centering
 \includegraphics[width=0.4\textwidth]{fig/network/fig1_2.pdf}
 \vspace{-4mm}
 \caption{
 xxxxxxxxx}
 \label{fig: Network FlowChart2}
\end{figure}
%

%
Specifically, assuming that the multi-scale features $\{E_i\}_{i=1}^s$ are from the encoder module of the U-Net in the diffusion model, where $s$ denotes a the number of scales, we first extract the multi-scale features $\{F_i\}_{i=1}^s$ from the short-exposure image by a feature extraction network\footnote{The details about the feature extraction network are included in the supplemental material.}, where the spatial resolution of $F_i$ is the same as $E_i$.  
%to guide $\{D_{i}\}_{i=1}^{s}$ in the diffusion process:
%\begin{equation}
%    \Tilde{D}_i =  \mathcal{C}(F_{(i)}, D_{(i)}), 
%    \label{eq:feature-fusion-cat}
%\end{equation}
%Then, with the estimated confidence map $M$, 
Then, with the multi-scale features $\{F_{i}\}_{i=1}^{s}$ and the estimated confidence map $M$, we develop a ExpBFusion, a simple yet effective feature fusion method, to guide $\{E_{i}\}_{i=1}^{s}$ in the diffusion process:
\begin{equation}
\begin{split}
    D_i = \mathcal{S}\left(\frac{\mathcal{Q}(\Tilde{D}_i)\mathcal{K}(\Tilde{D}_i)^\top}{\gamma}\right)\mathcal{V}(\Tilde{D}_i),
    \label{eq:feature-fusion}
    \end{split}
\end{equation}
where $\Tilde{D}_i = \mathcal{C}(F_i\otimes M_i, E_i\otimes M_i)$; $\mathcal{C}(\cdot)$ denotes a concatenation operation along the channel dimension; $M_i$ denotes the nearest downsmpling result of $M$, which has the same spatial resolution as $F_i$; $\otimes$ denotes the element-wise product operation; $\mathcal{Q}(\cdot)$, $\mathcal{K}(\cdot)$, and $\mathcal{V}(\cdot)$ denote the operations for extracting the query, key, and value matrices, respectively; $\gamma$ is a learnable weight parameter. 
%
Finally, we use the fused feature $D_i$ instead of $E_i$ in the diffusion process. 
%
We employ StableDiffusion-XL (SDXL) as our diffusion model as our diffusion model as it generates high-quality and realistic images
%











==> sec/4_experiments.tex <==


%
\begin{table}[!t]\footnotesize
\caption{Quantitative evaluations on the LSLB dataset. All the comparison results are generated using the publicly available code and trained on the same training datasets for fair comparisons. The number of NIQE, CLIPIQA+, and MUSIQ-PAQ2PIQ are tested on images of size $512 \times 512$ with locally blurred. The ``*'' represents that we concat the $\mathcal{N}_{s}$ and $\mathcal{B}_{l}$ as the model input, and ``$\downarrow$'' represents the values lower the results better.}
    \begin{tabular}{lcccc}
    \hline
    Methods         &NIQE $\downarrow$          &CLIPIQA+           &MUSIQ-PAQ2PIQ        \\ \hline
    MIMO-UNet~\cite{MIMO}       &9.9320                     &0.3130             &59.8464              \\
    NAFNet~\cite{NAFNet}          &9.2736                     &0.3045             &59.7057              \\
    Restormer~\cite{Restormer}       &9.6038                     &0.3051             &60.7811              \\
    % FftFormer       &                           &                   &                     \\
    MIMO-UNet*~\cite{MIMO}      &8.2208                     &0.2950             &63.6510              \\
    NAFNet*~\cite{NAFNet}          &8.2431                     &0.2977             &63.6596              \\
    Restormer*~\cite{Restormer}      &8.5662                     &0.3127             &64.7834              \\
    % FftFormer*      &                           &                   &                     \\
    % Selfir          &                           &                   &                     \\
    LBAG~\cite{RoLeBlur}            &10.0196                    &0.2968             &58.5612              \\
    % LMD-ViT         &                           &                   &                     \\
    Ours            &\textbf{4.6730}            &\textbf{0.3571}    &\textbf{65.3015}      \\ \hline
\end{tabular}
\label{compare1}
\end{table}
%
\begin{table}[!t]\small
\caption{Quantitative evaluations of the proposed approach against state-of-the-art methods on the ReLoBlur synthetic dataset. All the comparison results are generated using the publicly available codes and the models trained on the same training datasets.}
    \begin{tabular}{lcccc}
    \hline
    Methods                     &NIQE $\downarrow$          &CLIPIQA+           &MUSIQ-PAQ2PIQ        \\ \hline
    MIMO-UNet~\cite{MIMO}       &6.1947                     &0.3525             &58.0449              \\
    NAFNet~\cite{NAFNet}        &5.9387                     &0.3631             &59.9376              \\
    Restormer~\cite{Restormer}  &6.1146                     &0.3596             &59.2634              \\
    MIMO-UNet*~\cite{MIMO}      &5.9514                     &0.3607             &60.9325              \\
    NAFNet*~\cite{NAFNet}       &5.8419                     &0.3644             &61.2459              \\
    Restormer*~\cite{Restormer} &5.8826                     &0.3669             &61.4244              \\
    LBAG~\cite{RoLeBlur}        &5.9243                     &0.3644             &60.1322              \\
    LMD-ViT~\cite{LMD-ViT}      &5.9341                     &0.3389             &59.8619              \\
    Ours                        &\textbf{-}                 &\textbf{-}         &\textbf{-}           \\ \hline
\end{tabular}
\label{compare2}
\end{table}
%

%
\section{Experimental Results}
%
We evaluate the effectiveness of the proposed method against the state-of-the-art ones using public benchmark datasets.
%
\subsection{Experimental settings}
{\flushleft \textbf{Training datasets.}}
%
We use the RoLeBlur dataset~\cite{RoLeBlur} as our training dataset.
%
To generate short-exposure images, we first convert the sharp images into the hue saturation value (HSV) color space to reduce the brightness and add random noise to these images. 
% To generate short-exposure images, we first convert the sharp images into the Hue-Saturation-Value (HSV) color space and reduce the brightness by scaling down the V (Value) channel with a random factor between 0.25 and 0.3 to obtain a brightness-adjusted image. 
%
% Subsequently, we add random noise to these images to produce the final short-exposure images.
%
% Then, we crop the local motion blur image, ground-truth local blur mask, short-exposure images, and sharp image provided by RoLeBlur with the spatial size of 512 $\times$ 512 pixels.
Then we crop the input images and the corresponding masks with the spatial size of $512 \times 512$ pixels to focus on local details. 
%
We split the dataset into 19,351 pairs for training and 3,824 for evaluation.
%
To demonstrate the generalization ability of our proposed method on real-world data, we capture the real local motion blurred dataset LMBD that contains 10,380 images for training and 209 images for evaluation with smart phones. The details are included in the supplemental material.  
%
%Our proposed method is trained on the LSLB dataset and follows the protocol of existing methods for fair comparison.
%
%To demonstrate the robustness of the model, we synthesized a noisy short-exposure image using the ground truth from the ReLoBlur dataset, which we refer to as the ReLoBlur synthetic dataset. 
%
%We then conducted comparisons with existing methods based on this synthetic dataset.
%
%Since most handheld devices come with camera ISPs with anti-shake capability and anti-shake motor hardware support, most manufacturers focus on deblurring images with local blur caused by object motion, as these situations typically occur in real-world applications. 
%
%However, most existing synthetic deblurring datasets~\cite{REDS, RealWorld, DVD} tend to have heavy global blur due to their synthetic approach.
%
%Models trained on these datasets often do not handle blurry images with local blur well, and loss of detail in clear areas.
%
%To overcome this problem, we captured a  Long- and short-exposure local blur (LSLB) dataset through the main camera of the vivo X100 Pro as a training dataset.
%
%We capture the $B_{l}$ first, followed immediately by $N_{s}$. 
%
%To make the clear part of the image pleasantly, we make the shooting parameters of the $B_{l}$ default to the parameters of the camera, and we set the shooting parameters of the $N_{s}$ to 2.5ms in order to capture the motion objects.
%
%Specifically, we first select clear-noise data pairs based on the shot dataset, after which we generate masks of random areas, and exchange the corresponding mask partition in the clear image with the noise image as degraded images.
%
%After that, we use this data to train model~\cite{Resshift}. 
%
%We do the same operation for the clear and local blur data pairs and use the model trained on the clear-noise data to generate the corresponding gt for the local blur images.
%
%In summary, the LSLB dataset contains 10380 images for training and 100 images for testing.
%
%Our proposed method is trained on the LSLB dataset and follows the protocol of existing methods for fair comparison.
%
%To demonstrate the robustness of the model, we synthesized a noisy short-exposure image using the ground truth from the ReLoBlur dataset, which we refer to as the ReLoBlur synthetic dataset. 
%
%We then conducted comparisons with existing methods based on this synthetic dataset.

%
{\flushleft \textbf{Parameter settings.}}
% 
We implement our method using the PyTorch framework and train it on a machine with 8 NVIDIA GeForce RTX 4090 GPUs. 
%
The AdamW~\cite{adamw} optimizer with default parameters is used. The patch size is set to be $256 \times 256$ pixels, and the batch size is 32. 
%
We employ the loss function~\cite{PASD} to regularize our network and train the proposed network with 160,000 iterations, The initial learning rate is set to $5 \times 10^{-5}$.
%

%
%We set mixed precision to Half-precision floating-point and enable xformers-memory-efficient-attention to save memory on the GPU.
%
%Inspired by the structure of ControlNet, DLDN employs RealVisXL, which is a variant of StableDiffusion-XL (SDXL)~\cite{SDXL} aimed at photorealism.
%
{\flushleft \textbf{Evaluation metrics.}}
How to better evaluate the quality of restored images is important. Note that conventional distortion measures, e.g., PSNR and SSIM do not measure the visual quality of images well~\cite{tpdp}. We mainly use NIQE, CLIPIQA+, and MUSIQ-PAQ2PIQ as the main evaluation metrics as they are able to measure the visual quality of images well. 
%
\subsection{Comparisons with the state of the art}
%
We compare with the state-of-the-art method LBAG~\cite{RoLeBlur} in terms of local blur. 
%
To provide a comprehensive evaluation, we also compare it with global deblurring methods such as NAFNet~\cite{NAFNet}, Restormer~\cite{Restormer}, and MIMO-UNet~\cite{MIMO}.
%
As the proposed method requires a short-exposure image as guidance, one may wonder whether the performance gains are due to the use of additional information. To answer this question, we further use the concatenation of the blurry image and the short-exposure image as input of the existing methods for comparison. 
%
For fairness, we retrain the evaluated methods on the same training datasets and choose the best results for comparisons.
%
{\flushleft \textbf{Evaluations on the LMBD dataset.}} 
%
Table~\ref{compare1} shows the quantitative evaluation results.
%
Our method achieves the highest quantitative results.
%
Compared with global deblurring methods, our method shows a NIQE gain of at least 4.6 better than NAFNet~\cite{NAFNet}.
%
The above methods use the short-exposure image as the reference, which demonstrate measurable enhancements in their quantitative performance metrics compared to when reference image guidance is no provided.
%
However, the MUSIQ-PAQ2PIQ gain of our method is at least 0.52 higher than Restormer*~\cite{NAFNet} and 6.74 higher than local deblurring method LBAG~\cite{RoLeBlur}.
% %
% The proposed method generates the results with the highest CLIPIQA+ and MUSIQ-PAQ2PIQ and the lower NIQE values.
% %
% We use a single long-exposure image as input and a long-exposure image concat with a short-exposure image as inputs, respectively, in order to make a fair comparison with our method.
% %
% Compared to the Restormer method, which primarily targets globally blurred images, our method shows a NIQE gain at least 4.9308 lower than Restormer when using a single long-exposure image as input. When both long- and short-exposure images are used as inputs, our method's NIQE gain is at least 3.8932 lower than that of Restormer.
% %
% Compared to a local deblurring method ReLoBLur, our method generates the results with lower NIQE values.
%

%% Visual Comparisons
\begin{figure*}[t]
	\footnotesize
	\begin{center}
		\begin{tabular}{c c c c c c c c}
        \multicolumn{3}{c}{\multirow{5}*[48pt]{
            \hspace{-2.5mm} \includegraphics[width=0.42\linewidth,height=0.245\linewidth]{fig/experiments/1/fullimage.pdf}}}
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/1/input.pdf}
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/1/ReLoBlur.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/1/MIMO-UNet.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/1/NAFNet.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/1/Restormer.pdf} 
              \\
    		\multicolumn{3}{c}{~}                                   
            & \hspace{-4.0mm} (a) LQ
            & \hspace{-4.0mm} (b) ReLoBlur~\cite{RoLeBlur} 
            & \hspace{-4.0mm} (c) MIMO-UNet~\cite{MIMO}
            & \hspace{-4.0mm} (d) NAFNet~\cite{NAFNet} 
            & \hspace{-4.0mm} (e) Restormer~\cite{Restormer} 
            \\		
    	\multicolumn{3}{c}{~}
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/1/MIMO-UNet-cat.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/1/NAFNet-cat.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/1/Restormer-cat.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/1/ours.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/1/gt.pdf}
            \\
    	\multicolumn{3}{c}{\hspace{-4.0mm} \textbf{Blurry input}}
            & \hspace{-4.0mm} (f) MIMO-UNet*~\cite{MIMO} 
            & \hspace{-4.0mm} (g) NAFNet*~\cite{NAFNet} 
            & \hspace{-4.0mm} (h) Restormer*~\cite{Restormer}
            & \hspace{-4.0mm} (i) our
            & \hspace{-4.0mm} (j) GT patch\\ 	 	
        
		\end{tabular}
	\end{center}
 
	\vspace{-6mm}
	\caption{Visual comparisons on challenging \textbf{coupled degradation} inputs from the proposed benchmark. Zoom in for a better view.}
	\label{fig:visual1}
	%\vspace{-2mm}
\end{figure*}

%
Figure~\ref{fig:visual1} shows some visual comparisons of the evaluated methods.
%
The global deblurring methods do not remove the blur effects, as shown in Figure~\ref{fig:visual1}(c)-(e).
%
Figure~\ref{fig:visual1}(f)-(h) are the visual results of the above methods that use the short-exposure image as a reference and are still missing structural information.
% %
% Figure~\ref{fig:visual1} shows some visual comparisons of the evaluated methods. The methods NAFNet~\cite{NAFNet}, Restormer~\cite{Restormer}, and MIMO-UNet~\cite{MIMO} do not remove the blur effects as shown in Figure~\ref{fig:visual1}(b)-(e).
% %
% Figure~\ref{fig:visual1}(f)-(h) are the visual results of the above methods that use the concatenation of the blurry image and the short-exposure image as input.
% %
% However, the restored images still missing structural information.
%

%% Visual Comparisons
\begin{figure*}[t]
	\footnotesize
	\begin{center}
		\begin{tabular}{c c c c c c c c}	
        \multicolumn{3}{c}{\multirow{5}*[48pt]{
            \hspace{-2.5mm} \includegraphics[width=0.42\linewidth,height=0.245\linewidth]{fig/experiments/2/fullimage2.pdf}}}
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/2/input.pdf}
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/2/ReLoBlur.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/2/MIMO-UNet.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/2/NAFNet.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/2/Restormer.pdf} 
              \\
    		\multicolumn{3}{c}{~}                                   
            & \hspace{-4.0mm} (a) LQ
            & \hspace{-4.0mm} (b) ReLoBlur~\cite{RoLeBlur} 
            & \hspace{-4.0mm} (c) MIMO-UNet~\cite{MIMO}
            & \hspace{-4.0mm} (d) NAFNet~\cite{NAFNet} 
            & \hspace{-4.0mm} (e) Restormer~\cite{Restormer} 
            \\		
    	\multicolumn{3}{c}{~}
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/2/MIMO-UNet-cat.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/2/NAFNet-cat.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/2/Restormer-cat.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/2/our.pdf} 
            & \hspace{-4.0mm} \includegraphics[width=0.11\linewidth]{fig/experiments/2/gt.pdf}
            \\
    	\multicolumn{3}{c}{\hspace{-4.0mm} \textbf{Blurry input}}
            & \hspace{-4.0mm} (f) MIMO-UNet*~\cite{MIMO} 
            & \hspace{-4.0mm} (g) NAFNet*~\cite{NAFNet} 
            & \hspace{-4.0mm} (h) Restormer*~\cite{Restormer}
            & \hspace{-4.0mm} (i) our
            & \hspace{-4.0mm} (j) GT patch\\ 	 	
        
		\end{tabular}
	\end{center}
 
	\vspace{-6mm}
	\caption{Visual comparisons on challenging \textbf{coupled degradation} inputs from the proposed benchmark. Zoom in for a better view.}
	\label{fig:visual2}
	%\vspace{-2mm}
\end{figure*}

%
In contrast to the above methods, we utilize the priors from diffusion models to assist in the restoration of blurred regions to achieve a refinement effect in the blurred regions.
%
Thus, the deblurred results contain clear structures, and the hub of the tire and the ground appear much clearer as shown in Figure~\ref{fig:visual1}(i).
%

%
{\flushleft \textbf{Evaluations on the ReLoBlur synthetic dataset.}}
% We further evaluate our method on the ReLoBlur synthetic dataset that contains 19351 patch pairs for training and 3824 patch pairs for the test.
%
% We employ the same validation method as the one used in the ReLoBlur dataset for fair comparisons.
%
Table~\ref{compare2} summarizes the quantitative evaluation results, where the proposed method achieves high-quality results with higher NIQE, CLIPIQA+, and MUSIQ-PAQ2PIQ values. 
%
Although the global deblurring methods use short-exposure images as reference (e.g., Restormer*~\cite{Restormer}), they show improvement in the results compared to when no reference image guidance, the NIQE gain of our method is at least \yzb{XXXX} better than above methods.
%

%
Figure~\ref{fig:visual2} shows a visual comparison,  we observe that the evaluated methods do not restore the bicycle basket effectively, with the mathod~\cite{Restormer} showing color biases. In contrast, our method generates better results.
%
For example, the bicycle basket is much clearer.
%

==> sec/5_abalation.tex <==
%
\begin{table*}[!t]
\caption{Quantitaive evaluations of each component in the proposed method on the LSLB dataset.}
\label{tab:abation}
\begin{tabular}{lcccccccc}
\hline
                                        &~~BMSSAM~~        &~~MGF~~         &~~GF~~           &~~DBDM~~      &~~NIQE $\downarrow$~~     &~CLIPIQA+~           &~~MUSIQ-PAQ2PIQ~~            \\ \hline
DLDNet$_{\text{w/o MGF}}$               &\XSolidBrush      &\XSolidBrush    &\XSolidBrush     &\XSolidBrush  &5.8205                    &0.2815               &62.1051                      \\
DLDNet$_{\text{w/ GF}}$                 &\XSolidBrush      &\Checkmark      &\XSolidBrush     &\XSolidBrush  &6.8091                    &0.3296               &59.5076                      \\
DLDNet$_{\text{w MGF}}$                 &\XSolidBrush      &\Checkmark      &\XSolidBrush     &\Checkmark    &4.6861                    &0.3395               &62.4996                      \\
DLDNet$_{\text{w BMSSAM \& w/oMask}}$   &\XSolidBrush      &\XSolidBrush    &\Checkmark       &\XSolidBrush  &4.8490                    &0.3368               &64.7102                      \\
DLDNet                                  &\Checkmark        &\Checkmark      &\XSolidBrush     &\Checkmark    &\textbf{4.6730}           &\textbf{0.3571}      &\textbf{65.3015}             \\ \hline
\end{tabular}
\end{table*}
%

%
\section{Analysis and Discussion}
%
To better understand how our method addresses local motion deblurring with reference images, and demonstrate the effect of its main components, we provide in-depth analyses of the proposed method, For the ablation studies in this section, we train our method and all the baselines on the LSLB dataset using the batch size of 32 to illustrate the effect of each component in our method.   
% %
% Our experiments show that using mask guided image filtering in blurred areas to make blurred images capture structural information corresponding to short-exposure images generates favorable results and advantages over state-of-the-art methods. 
% %
% In this section, we analyze the proposed methodology and show the effects of the main components.
% %
% For the ablation studies in this section, we train our method and all baseline methods on the LSLB dataset.
% %
% The batch size is set to 32 to illustrate the effect of each component in our method.
%
\subsection{Blurry-aware guided image restoration}
\label{ablation51}
%
The proposed blurry-aware guided image restoration is used to eliminate blur with the guidance of a short-exposure image in blurred regions.
%
To demonstrate the effectiveness of the blurr-aware guided image restoration we proposed, we first compare the baseline that only long-exposure image is used to guide the restoration of the locally blurred image (DLDNet$_{\text{w/o MGF}}$ for short) with the apply guided image filtering to both long-exposure locally blurred image and the short-exposure image without using blurry regions mask (DLDNet$_{\text{w/ GF}}$ for short) and train them using the same setting on the LSLB dataset for fair comparisons.

% To demonstrate the effectiveness of the Blurry-aware guided image restoration we proposed, we first do not use the short-exposure image to guide the restoration of the locally blurred image (DLDNet$_{\text{w/o MGF}}$ for short).
% %
% Mask Guided image filtering is proposed to restore localized blurring image better by using a short-exposure image to guided localized blur corresponding to a locally blurred image: a short-exposure image-guided localized blur.
% %
% To demonstrate the effectiveness of the Mask Guided image filtering we proposed, We first do not use the short-exposure image to guide the restore of the locally blurred image (DLDNet$_{\text{w/o MGF}}$ for short). 
% %
% Based on this, we apply guided filtering to the locally blurred image and the short-exposure image without using a mask (DLDNet$_{\text{w/ GF}}$ for short).
%
Table~\ref{tab:abation} shows that DLDNet$_{\text{w/o GF}}$ generates better deblurring results compared to the baseline, with the CLIPIQA+ and MUSIQ-PAQ2PIQ values for DLDNet$_{\text{w/ GF}}$ are 0.0481 and 1.1086dB higher, respectively, than DLDNet$_{\text{w/o MGF}}$. 
%
To address the issue mentioned in section~\ref{sec:MGIF}, where directly using~\cite{GIF} smooths the clear background of long-exposure images, we incorporate a blurred regions mask based on the method DLDNet$_{\text{w/o MGF}}$ (DLDNet$_{\text{w MGF}}$ for short).
%
The results in Table~\ref{tab:abation} show that using the blurred regions mask as a prior with guided image filtering generates better results, where the CLIPIQA+ and MUSIQ-PAQ2PIQ values are 0.01 and 0.3945 higher.
%

%
\begin{table}[!t] 
\centering
\label{tab:DBDN}
\caption{Effect of the proposed DBDN on the LSLB dataset.The ``CP'' denotes the Confidence Predictor in LDM-ViT~\cite{LMD-ViT}}
\begin{tabular*}{\linewidth}{lcc}
\hline
Methods                      &~~~~~~~~~~~~~~~~~ACC~~~~~~~             &~~~~~~~MIOU~~~~~~~                  \\ \hline
CP                           &                                        &                                    \\
DBDM                         &                                        &                                    \\ \hline              
\end{tabular*}
% }
\vspace{-3mm}
\end{table}
%

%
Figure~\ref{fig:ablation_1} shows the visualization results by these above mentioned methods. 
%
Using the proposed blurry-aware guided image restoration generates better deblurred images,  where the car tail recovered well shown in Figure~\ref{fig:ablation_1}(c).
%
Using the guided image filtering method has a slight deblur effect but thestatic bike and the ground appeared smooth as well shown in Figure~\ref{fig:ablation_1}(b).
%

\subsection{Short-exposure guided diffusion model}
\label{ablation52}
%
The proposed MSSAM is used to provide a prompt that describes the structural details of the blurred area more accurately than the text prompt during the diffusion generation process.
%
To demonstrate its effectiveness for the image generation process of DLDNet, we add the BMSSAM to DLDNet$_{\text{w MGF}}$ (DLDNet for short).
%
Table~\ref{tab:abation} shows that combining the masks of short-exposure images and blurred images as prompts to guide the diffusion process using BMSSAM generates better results, where the CLIPIQA+ and PSNR value are 0.0176 and \yzb{xxx} higher.
%

%
Figure~\ref{fig:ablation_2} shows the visualization results by these above mentioned methods. 
%
Using the proposed BSSAM generates better deblurred images, where the lines of the tires and the ground in the background are more defined.
%
\begin{figure}[h] %\footnotesize
\centering
  \begin{tabular}{ccc}
        \includegraphics[width=0.3\linewidth]{fig/ablation/ablation_gf/woGF.pdf} &\hspace{-3mm}
        \includegraphics[width=0.3\linewidth]{fig/ablation/ablation_gf/wGF.pdf} &\hspace{-3mm}
        \includegraphics[width=0.3\linewidth]{fig/ablation/ablation_gf/wMGF.pdf} \\
        (a) DLDNet$_{\text{w/o MGF}}$ &\hspace{-3mm} 
        (b) DLDNet$_{\text{w/ GF}}$ &\hspace{-3mm}  
        (c) DLDNet$_{\text{w MGF}}$ \\

    \end{tabular}
    \caption{ Effectiveness of the proposed blurry-aware guided image restoration on image deblurring.}
    \label{fig:ablation_1}
\end{figure}
%
\begin{figure}[h] %\footnotesize
\centering
  \begin{tabular}{ccc}
        \includegraphics[width=0.3\linewidth]{fig/ablation/ablationBMSSAM/woMSSM_patch.pdf} &\hspace{-5mm}
        \includegraphics[width=0.3\linewidth]{fig/ablation/ablationBMSSAM/MSSMwoMask_patch.pdf} &\hspace{-5mm}
        \includegraphics[width=0.3\linewidth]{fig/ablation/ablationBMSSAM/ours_patch.pdf} \\
        (a) DLDNet$_{\text{w/o MGF}}$  &\hspace{-5mm} 
        (b) DLDNet$_{\text{w/ BSSAM}}$    &\hspace{-5mm}  
        (c) DLDNet                      \\

    \end{tabular}
    \caption{ Effectiveness of the proposed BMSSAM on image deblurring.}
    \label{fig:ablation_2}
\end{figure}
%
\begin{figure}[h] %\footnotesize
\centering
  \begin{tabular}{ccc}
        \includegraphics[width=0.3\linewidth]{fig/ablation/ablationBMSSAM/wMGF1111.png} &\hspace{-5mm}
        \includegraphics[width=0.3\linewidth]{fig/ablation/ablationBMSSAM/BSSAMwoMask1111.png} &\hspace{-5mm}
        \includegraphics[width=0.3\linewidth]{fig/ablation/ablationBMSSAM/Our1111.png} \\
        (a) DLDNet$_{\text{w/o MGF}}$  &\hspace{-5mm} 
        (b) DLDNet$_{\text{w/ BSSAM}}$    &\hspace{-5mm}  
        (c) DLDNet                      \\

    \end{tabular}
    \caption{ Effectiveness of the proposed DBDM on image deblurring.}
    \label{fig:ablation_3}
\end{figure}
%

%
\subsection{Effect of DBDM}
%
To demonstrate the effectiveness of the proposed blurred regions detection module in identifying blurred areas within locally blurred images, We first use the DBDM to generate masks, replacing the ground truth masks in the DLDNet.
%
The result in Table~\ref{tab:abation} shows that using the mask generated by DBDM does not perform poorly with the ground truth one,
%
Then we compare DBDM with the Confidence Predictor in LDM-ViT~\cite{LMD-ViT} on the LSLB dataset.
%
We use the accuracy (ACC) and Mean Intersection over Union (MIOU) as metrics to evaluate the quality of the capability of identifying blurred regions.
%
Table~\ref{tab:DBDN} shows that the DBDM identifies the blur aware with higher ACC and MIOU values, where the ACC and MIOU values of the DBDM are at least \yzb{xxx} and \yzb{xxx} higher than Confidence Predictor on the LSLB dataset.
%

%
Figure~\ref{fig:ablation_3} shows visual comparisons of the DBDM and the Confidence Predictor.
%
The Confidence Predictor mistakenly classifies clear pixels as blurred.
%
However, the mask generated by DBDM has high accuracy and can effectively cover the blurred regions.




% %
% \begin{table}[!t]\scriptsize
% \caption{Effect of the proposed blurry-aware aguded image restoration in the proposed method on the LMBD dataset.}
% \label{tab:abation}
% \begin{tabular}{lcccccc}
% \hline
%                         &~~~~~~GF                & $M$                     &~~NIQE $\downarrow$         &CLIPIQA+             &MUSIQ-PAQ2PIQ       \\  \hline
% ${\text{w/o MGF}}$      &\XSolidBrush      &\XSolidBrush            &5.8205                    &0.3296               &62.1051                      \\
% ${\text{w/ GF}}$        &\Checkmark        &\XSolidBrush            &6.8091                    &0.2815               &59.5076                      \\
% $\text{w/ MGF}$         &\Checkmark        &\Checkmark              &4.6861                    &0.3395               &62.4996                      \\  \hline
% \end{tabular}
% \end{table}
% %

% %
% \begin{table}[!t]\scriptsize
% \caption{Effect of proposed ExpBFusion in the proposed method on the LMBD dataset.}
% \label{tab:abation}
% \begin{tabular}{lcccccc}
% \hline
%                                           &Fusion                       & $M$                      &NIQE $\downarrow$         &CLIPIQA+                  &MUSIQ-PAQ2PIQ                \\ \hline
% ${\text{w/o Fusion}}$                     &\XSolidBrush                 &\XSolidBrush              &4.6861                    &0.3395                    &62.4996                      \\                     
% ${\text{\& w/o M}}$                       &\Checkmark                   &\XSolidBrush              &4.8490                    &0.3368                    &64.7102                      \\
% ExpRDiff                                  &\Checkmark                   &\Checkmark                &\textbf{4.6730}           &\textbf{0.3571}           &\textbf{65.3015}             \\ \hline
% \end{tabular}
% \end{table}
% %

% %
% \begin{table}[!t]\scriptsize
% \caption{Effect of proposed DBDM in the proposed method on the LMBD dataset.}
% \label{tab:abation}
% \begin{tabular}{lcccccc}
% \hline
%                             &DBDM                & $M^{gt}$              &NIQE $\downarrow$         &CLIPIQA+             &MUSIQ-PAQ2PIQ                \\ \hline
% ${\text{w/ DBDM}}$          &\XSolidBrush        & \XSolidBrush          &4.8490                    &0.3368               &64.7102                      \\                     
% ${\text{w/ M}^{gt}}$        &\XSolidBrush        & \Checkmark            &-                         &-                    &-                            \\
% ExpRDiff                    &\Checkmark          & \XSolidBrush          &\textbf{4.6730}           &\textbf{0.3571}      &\textbf{65.3015}             \\ \hline
% \end{tabular}
% \end{table}
% %

%
% \begin{table*}[!t]
% \caption{Quantitaive evaluations of each component in the proposed method on the LMBD dataset.}
% \label{tab:abation}
% \begin{tabular}{lcccccccc}
% \hline
%                                           &~~BMSSAM~~        &~~MGF~~         &~~GF~~           &~~DBDM~~           &~~NIQE $\downarrow$~~     &~CLIPIQA+~           &~~MUSIQ-PAQ2PIQ~~            \\ \hline
% ExpRDiff$_{\text{w/o MGF}}$               &\XSolidBrush      &\XSolidBrush    &\XSolidBrush     &\XSolidBrush       &5.8205                    &0.3296               &62.1051                      \\
% ExpRDiff$_{\text{w/ GF}}$                 &\XSolidBrush      &\Checkmark      &\XSolidBrush     &\XSolidBrush       &6.8091                    &0.2815               &59.5076                      \\
% ExpRDiff$_{\text{w MGF}}$                 &\XSolidBrush      &\Checkmark      &\XSolidBrush     &\Checkmark         &4.6861                    &0.3395               &62.4996                      \\
% ExpRDiff$_{\text{w BMSSAM \& w/oMask}}$   &\XSolidBrush      &\XSolidBrush    &\Checkmark       &\XSolidBrush       &4.8490                    &0.3368               &64.7102                      \\
% ExpRDiff$_{\text{w M}^{gt}}$              &\XSolidBrush      &\XSolidBrush    &\Checkmark       &\XSolidBrush       &-                         &-                    &-                      \\
% ExpRDiff                                  &\Checkmark        &\Checkmark      &\XSolidBrush     &\Checkmark         &\textbf{4.6730}           &\textbf{0.3571}      &\textbf{65.3015}             \\ \hline
% \end{tabular}
% \end{table*}
%

==> sec/6_conclusion.tex <==
%
\section{Conclusion}
%
We propose ExpRDiff to explore features from short-exposure images and blurry regions to guide local blur removal and realistic image restoration.
%
To improve the identification of blurry regions, we design a context-based local blur detection module that incorporates additional contextual information to determine whether the regions are blurry or not.
%
Subsequently, we develop a blur-aware guided image restoration method that utilizes sharp structural details from short-exposure images, facilitating accurate reconstruction of heavily blurred regions.
%
Furthermore, to achieve realistic images with better visually appealing restoration, we present a short-exposure guided diffusion model that utilizes features from both short-exposure images and blurred regions to effectively guide the diffusion process.
%
Experimental results show that \ournet performs favorably against the state-of-art methods.
%

